Approximation with Random Shallow ReLU Networks with Applications to Model Reference Adaptive Control

Neural networks are regularly employed in adaptive control of nonlinear systems and related methods of reinforcement learning. A common architecture uses a neural network with a single hidden layer (i.e. a shallow network), in which the weights and biases are fixed in advance and only the output layer is trained. While classical results show that there exist neural networks of this type that can approximate arbitrary continuous functions over bounded regions, they are non-constructive, and the networks used in practice have no approximation guarantees. Thus, the approximation properties required for control with neural networks are assumed, rather than proved. In this paper, we aim to fill this gap by showing that for sufficiently smooth functions, ReLU networks with randomly generated weights and biases achieve $L_{\infty}$ error of $O(m^{-1/2})$ with high probability, where $m$ is the number of neurons. It suffices to generate the weights uniformly over a sphere and the biases uniformly over an interval. We show how the result can be used to get approximations of required accuracy in a model reference adaptive control application.

==> background.tex <==
\section{Background on Function Approximation with Neural Networks}
\label{sec:apx:background}
Let $\Cs(\Bc)$ be the set of continuous functions $f:\Bc\to \R$, where $\Bc$ is a bounded set containing the origin. 


Formally, for a given target function $f\in \Cs(\Bc)$, positive integer $N\in\N$, and positive 
scalar $\epsbase>0$ (which may depend on $N$) there exists some vector $\theta\in\R^N$ and 
nonlinear, continuous almost everywhere basis functions $\Bs_1,\dots,\Bs_N:\R^n\to\R$ such that 
the approximation
\begin{equation}\label{eq:apx:genApx}
\fh(x) \ := \ \sum_{i=1}^N \theta_i\,\Bs_i(x)
%\approx f(x) \hspace{40pt}\forall x\in\Bc
\end{equation}
satisfies
\begin{equation}\label{eq:apx:normBound}
%\sup_{x\in\Bc}\abs{f(x)-\fh(x)} \leq \epsbase
%\qquad\text{or}\qquad
\normB{\fch(x)-\fh(x)} \ \leq \ \epsbase \ \ .
\end{equation}
Here, we denote the the $L_2(\Bc,\muB)$ norm
$$
\normB{\fch(x)} \ := \ \left(\int_B|\fch(x)|^2\,\muBdx\right)^{\frac{1}{2}}
$$
with $\muB$ as the uniform probability measure over $\Bc$ such that $\int_\Bc\muBdx=1$, and some
\textit{affine shift} $\fch(x)=f(x)-\mathscr{a}^\top\!x -\mathscr{b}$, for some 
$\mathscr{a}\in\R^n$ and $\mathscr{b}\in\R$.
% (typically $\mathscr{a}=\nabla f(0)$ and $\mathscr{b}=f(0)$).

Throughout the paper, we will assume that $\sigma$ is the ReLU activation function:
\begin{equation}
  \label{eq:relu}
  \sigma(t)=\max\{0,t\}.
\end{equation}

We will assume that the basis function is parameterized $\Bs(x\,;\upgamma)$ and is a 
composition of some nonlinear, continuous almost everywhere function $\sigma:\R\to\R$ together
with an affine transformation of $\R^n$ into $\R$ according to the \textit{parameter} 
$\upgamma\in\Upsilon$. We define each point $\upgamma:=[w^\top\ b]^\top=[w_1\ \dots\ w_n\ 
b]^\top$ with $w\in\R^n\setminus\{0_n\}$ as the \textit{weight vector} and $b\in\R$ as the
\textit{bias term}. We assume the \textit{parameter set} $\Upsilon$ is a bounded subset of 
$\R^n\setminus\{0_n\}\times\R$. And so, we set $\Bs(x\,;\upgamma_i)=\sigma(w_i^\top 
x+b_i)=\sigma(\pariX)$, where 
$X:=[x_1\ \cdots\ x_n\ 1]^\top$ and we denote $\upgamma_i=[w_i^\top\ b_i]^\top=[w_{i,1}\
\dots\ w_{i,n}\ b_i]^\top$, for all $i\in[N]$. 

We will use the term \textit{base approximation} to define, for some vector $\theta\in\R^N$ and
\underline{fixed} parameters $\upgamma_1,\dots,\upgamma_N\in\Upsilon$, for any integer $N\in\N$,
the sum
\begin{equation}\label{eq:apx:baseApx}
\fhN(x) = \sum_{i=1}^{N} \theta_i\,\sigma(\pariX)
%\approx f(x) 
%\hspace{40pt}\forall x\in\Bc
\ \ ,
\end{equation}
and \textit{random approximation} to define, for
% is similarly constructed, but in this case the parameters are
%\textit{randomly sampled} from $\Upsilon$. Thus, it refers 
some vector $\vartheta\in\R^R$ and \textit{randomly sampled} parameters
$\upgammab_1,\dots,\upgammab_R\in\Upsilon$, for any integer $R\in\N$, the sum
\begin{equation}\label{eq:apx:rndApx}
\fhR(x\,;\upgammab_1,\dots,\upgammab_R) = \sum_{j=1}^{R}\vartheta_j\,\sigma(\parbjX)
%\approx f(x) \hspace{40pt}\forall x\in\Bc
\ \ .
\end{equation}
%Note that we use integer $R$ and index $j$ for random approximations to distinguish them
%from base approximations, but otherwise there is no significance.

Note that these linear combinations are equivalent to a feedforward 
neural network with a single hidden layer, as depicted in Figure~\ref{fig:apx:SHLNN}, wherw 
$x_0=1$. Hence why we refer to $\sigma$ as an \textit{activation function}, as the output of 
each neuron is the activation of the weighted inputs (plus bias term) to the neuron. We will 
assume that the activation function $\sigma$ is bounded (growth)
% over all feasible inputs$\parX$ in $\Upsilon\times\Bc\times\{1\}$, 
as follows.

\begin{figure}
\centering
\begin{tikzpicture}[x=1.2cm, y=0.75cm, >=stealth]

\foreach \m/\l [count=\y] in {1,2,missing,3}
  \node [every neuron/.try, neuron \m/.try] (input-\m) at (0,1.5-\y) {};

\foreach \m [count=\y] in {1,missing,2}
  \node [every neuron/.try, neuron \m/.try ] (hidden-\m) at (2,2.5-\y*1.75) {};

\foreach \m [count=\y] in {1}
  \node [every neuron/.try, neuron \m/.try ] (output-\m) at (4,0.1-\y) {};

%\foreach \l [count=\i] in {1}
%  \draw [<-] (input-\i) -- ++(-1,0)
%    node [above, midway] {$x_\l$};

\foreach \l [count=\i] in {0,1,n}
  \draw [<-] (input-\i) -- ++(-1,0)
    node [above, midway] {$x_\l$};

\foreach \l [count=\i] in {1,n}
  \node [above] at (hidden-\i.north) {$\sigma$};

\foreach \l [count=\i] in {1}
  \draw [->] (output-\i) -- ++(1,0)
    node [above, midway] {$\fh(x)$};

\foreach \i in {1,...,3}
  \foreach \j in {1,...,2}
    \draw [->] (input-\i) -- (hidden-\j);

\foreach \i in {1,...,2}
  \foreach \j in {1}
    \draw [->] (hidden-\i) -- (output-\j);

%\foreach \l [count=\x from 0] in {Input, Hidden, Ouput}
%  \node [align=center, above] at (\x*2,2) {\l \\ layer};

\node[] at (0.9,0.9) {$b_1$};
\node[] at (1.5,-1.4) {$b_N$};
\node[] at (0.8,0.3) {$w_{1,1}$};
\node[] at (1.0,-0.3) {$w_{1,n}$};
\node[] at (0.9,-2.0) {$w_{N,1}$};
\node[] at (1,-2.9) {$w_{N,n}$};
\node[] at (3,0.2) {$\theta_1$};
\node[] at (3,-2.3) {$\theta_N$};

\end{tikzpicture}
\caption{\label{fig:apx:SHLNN} Single hidden-layer neural network with $\sigma$ activation 
function.}
\end{figure}


\begin{assumption}\label{sigAsmpt}
\textit{
The nonlinear, continuous almost everywhere activation function $\sigma:\R\to\R$ is bounded 
(growth) over all feasible inputs, such that either of}
\begin{enumerate}
\item $|\sigma(u) - \sigma(v)| \ \leq \ \Dsig$
\item $|\sigma(u) - \sigma(v)| \ \leq \ \Lsig\,|u-v|$
\end{enumerate}
\textit{
hold for all $u,v\in\Ic:=\{\parX \ | \ (\upgamma,X)\in\Upsilon\times\Bc\times\{1\}\}$,
with positive scalar $\Dsig$ or $\Lsig$.}
\end{assumption}

If we shift the activation to the origin as $\sigmach(y):=\sigma(y)-\sigma(0)$, this maintains 
the assumption with the same constant in either case.
The (scaled) step function $\sstep$ and the ReLU function $\relu$, defined as
\begin{align}
\sstep(y) &= 
\begin{cases*}\label{eq:pe:step}
0 \quad\text{if } y\leq0 \\
c \quad\text{if } y>0
\end{cases*}
\qquad \text{(scaled step)} \\
\relu(y) &= 
\begin{cases*}\label{eq:pe:ReLU}
0 \quad\text{if } y\leq0 \\
y \quad\text{if } y>0
\end{cases*}
\qquad \text{(ReLU)} \ \ ,
\end{align}
are examples meeting Assumption~\ref{sigAsmpt}, with $\Dsig=c$ and $\Lsig=1$ respectively,
where $c>0$ is an arbitrary positive scalar.


 	
%%% Local Variables:
%%% TeX-master: "main.tex"
%%% End:


==> mollified.tex <==
\section{Mollified Approximations}
\label{sec:apx:mollApx}
In this section, we define the \textit{mollified approximation} $\fhlN$ using a novel method of 
forming a \textit{mollified integral representation} for a base approximation $\fhN$ to a 
target function $f\in\Cs(\Bc)$, and bound their difference in the $L_2(\Bc,\muB)$ norm.


\subsection{Functions with Integral Representation}
If a target function $f:\R^n\to\R$ has an \textit{integral representation} over the parameters
set $\Upsilon$ with some activation function $\sigma:\R\to\R$, then
\begin{equation}\label{eq:apx:intRep}
f(x) \ = \ \int_\Upsilon \gs(\upgamma)\,\sigma(\parX)\,\d\upgamma
% \hspace{40pt} \forall x\in\Bc
\end{equation}
holds with some bounded, continuous \textit{coefficient function} \mbox{$\gs:\Upsilon\to\R$}. 
This is a version of \eqref{eq:apx:baseApx} that is continuous in the parameters $\upgamma_i$ 
over $\Upsilon$. Indeed, if we define $\upgamma_1,\dots,\upgamma_N$ to be a sequence of points 
that uniformly grids $\Upsilon$ with volume $\d_N$ between any neighboring points, then as
$N\to\infty$ (and $\d_N\to0$) we have
$$
\lim\limits_{N\to\infty}\sum_{i=1}^{N}\gs(\upgamma_i)\,\sigma(\pariX)\,\d_N 
= \int_\Upsilon \gs(\upgamma)\,\sigma(\parX)\,\d\upgamma = f(x)
%\forall x\in\Bc
\ .
$$
This implies that the (infinite) sum of the absolute values of the coefficients is finite, with
$$
%C_\infty := 
\lim\limits_{N\to\infty}\sum_{i=1}^{N}|\gs(\upgamma_i)|\,\d_N \ 
= \ \int_\Upsilon |\gs(\upgamma)|\,\d\upgamma \ < \ \infty
$$
holding since $\gs$ is bounded and the integral is over the bounded set $\Upsilon$.

However, finding such integral representations \eqref{eq:apx:intRep} for general classes of
functions $f$ and activation functions $\sigma$ is a nontrivial task. If \textit{both}
are $L_1$ (absolutely integrable over $\R^n$ and $\R$ respectively), then Theorem 1 in
\cite{irie1988capabilities} shows that the integral representation can always be constructed
with $\gs$ related to the Fourier transforms of $f$ and $\sigma$. But this is a limiting
restriction, since none of the typical activation functions like sigmoids, steps, ReLU's, and 
their variants meet this requirement. Even so, in \cite{funahashi1989approximate} this was used 
to prove the universal approximation properties of sigmoid activations.
%In
%\cite{hsu2021approximation}, it is shown that a particular definition of a trigonometric ridge
%function has an integral representation with ReLU activations, and then those ridge functions
%can be the basis functions as in \eqref{eq:apx:genApx} for target functions in $L_2([-1,1]^n)$.
%But again, this is a limited class of target functions compared to $\Cs(\Bc)$.


\subsection{Mollified Integral Representation}
\label{sec:apx:moll}
Now we will propose a novel method of forming an integral representation for
\textit{any} function $f\in\Cs(\Bc)$, so long as a base approximation $\fhN$ of the form 
\eqref{eq:apx:baseApx} exists and the bounded parameter set $\Upsilon\subset\R^{n+1}$ and a
bound $\Sc_N$ on the coefficient size $\sum_{i=1}^N|\theta_i|$ are known.

For any fixed parameters $\upgamma_1,\dots,\upgamma_N\in\Upsilon$, this approximation $\fhN$ 
can be defined as
\begin{align}\nonumber
\fhN(x) \ =& \  \sum_{i=1}^{N} \theta_i\,\sigma(\pariX) \\\label{eq:apx:baseIntRep}
=& \ 
\int_\Upsilon \,\sum_{i=1}^N\theta_i\,\deltano(\upgamma-\upgamma_i)\ \sigma(\parX)\,\d\upgamma \ 
\ ,
\end{align}
where $\deltano$ is the $(n+1)$-dimensional Dirac delta which satisfies for any
$\upgamma_i\in\Upsilon$ that
$\int_\Upsilon\deltano(\upgamma-\upgamma_i)\,\sigma(\parX)\,\d\upgamma =\sigma(\pariX)\ $.

Thus, the RHS of \eqref{eq:apx:baseIntRep} is like an integral representation 
\eqref{eq:apx:intRep} of $\fhN$ with a coefficient mapping \mbox{$\gs(\upgamma) = \sum_{i=1}^N 
\theta_i\,\deltano(\upgamma-\upgamma_i)$}.
However, this mapping is not continuous and bounded as required, and the Dirac delta is not even
a function in the regular sense. Indeed, if the overall coefficients of a random approximation 
$\fhR$ were set as $\vartheta_j=\gs(\upgammab_j)$ for each randomly sampled 
$\upgammab_1,\dots,\upgammab_R\in\Upsilon$, then in this case they almost surely would all be 
zero.

We propose the \textit{Mollified integral representation} to solve this issue, where the Dirac
delta in \eqref{eq:apx:baseIntRep} is replaced with the \textit{mollified} delta function
$\deltalno$. Recalling that $\upgamma=[w_1\ \cdots\ w_n\ b\,]$, this is defined as the 
$(n+1)$-dimensional bump function
\begin{align}\label{eq:apx:mollDel}
&\deltalno(\upgamma) \ := \ \\\nonumber
&\begin{cases}
(\eta\lambda)^{n+1}\prod_{i=1}^n
\exp\left(\dfrac{-1}{1-\lambda^2w_i^2}\right)
%\cdots\,
%\exp\left(\dfrac{-1}{1-\lambda^2w_n^2}\right)\,
\exp\left(\dfrac{-1}{1-\lambda^2b^2}\right)\\[8pt]
\hspace{160pt} \upgamma\in(-\frac{1}{\lambda},\frac{1}{\lambda})^{n+1} \\
0 \hspace{155pt} \text{otherwise}
\end{cases}
\end{align}
with $\eta^{-1}=\int_{-1}^{1}\exp\left(\frac{-1}{1-y^2}\right)\d y \approx0.444$ thus giving
$\int\deltalno(\upgamma-\upgamma_i)\,\d\upgamma = \int\deltano(\upgamma-\upgamma_i)\,\d\upgamma
= 1$ for any $n\geq1$ and $\upgamma_i\in\R^{n+1}$.

We term the positive scalar $\lambda>0$ as the \textit{mollification factor}. This controls the
height and width of the \mbox{mollified} delta $\deltalno$. Since the height scales as
$\lambda^{n+1}$ and the integral remains constant, this requires the width to shrink. 
Figure~\ref{fig:apx:mollFactor} plots the 1-dimensional case for different $\lambda$ values.
%\begin{figure}[H]
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{mollFactor}
\caption{\label{fig:apx:mollFactor}The mollified delta $\deltal$ for different $\lambda$ values.
In each case, $\int_{-1/\lambda}^{1/\lambda}\deltal(\upgamma)\d\upgamma=1$.}
\end{figure}

The support of $\deltalno(\upgamma-\upgamma_i)$ is the $(n+1)$-dimensional open cube set
$(-\frac{1}{\lambda},\frac{1}{\lambda})^{n+1}$ centered about any $\upgamma_i\in\Upsilon$. And
so, if $\upgamma_i$ is sufficiently close to (or on) the boundary of $\Upsilon$, then it no
longer holds that the entire support of $\deltalno(\upgamma-\upgamma_i)$ is within $\Upsilon$.
Thus, we define the \textit{$\lambda$-expanded} parameters set $\Upsilonl$ such that the support
is always fully contained, up to and include the boundary of $\Upsilon$. For example, if
$\Upsilon$ is rectangular product of intervals $[\alpha_1,\beta_1]\times\cdots\times
[\alpha_n,\beta_n]$, then each interval is expanded as 
$[\alpha_i-\frac{1}{\lambda},\beta_i+\frac{1}{\lambda}]$ to obtain $\Upsilonl$.
With this $\lambda$-expanded parameters set, we always maintain that
$\int_\Upsilonl\deltalno(\upgamma-\upgamma_i)\d\upgamma=1$ for all $\lambda>0$, $n\geq1$, and any
$\upgamma_i\in\Upsilon$.

Since $\Upsilon\subset\Upsilonl$ for all $\lambda>0$, then \eqref{eq:apx:baseIntRep} is 
equivalently
\begin{equation}\label{eq:apx:baseIntRepLam}
\fhN(x) = \int_\Upsilonl \,\sum_{i=1}^N\theta_i\,\deltano(\upgamma-\upgamma_i)\ 
\sigma(\parX)\,\d\upgamma \ \ .
\end{equation}
And so, by replacing the Dirac delta in \eqref{eq:apx:baseIntRepLam} with the mollified delta
$\deltalno$, for any choice of $\lambda>0$, we obtain the corresponding \textit{mollified 
approximation}
\begin{equation}\label{eq:apx:mollApx}
\fhlN(x) := \int_\Upsilonl \,\sum_{i=1}^N\theta_i\,\deltalno(\upgamma-\upgamma_i)\ 
\sigma(\parX)\,\d\upgamma
\end{equation}
using a \textit{mollified integral representation}.
This now gives the required continuous, bounded coefficient mapping for any fixed
$\upgamma_1,\dots,\upgamma_N\in\Upsilon$ as
\begin{equation}\label{eq:apx:gLam}
\gl(\upgamma) := \sum_{i=1}^N\theta_i\,\deltalno(\upgamma-\upgamma_i)
%\ \leq \ \left(\frac{\eta\lambda}{e}\right)^{n+1}\sum_{i=1}^N|\theta_i|
\ \ .
\end{equation}
We illustrate the transformation for the 1-dimensional case conceptually in 
Figure~\ref{fig:apx:moll}.
%\begin{figure}[H]
\begin{figure}
\centering
\includegraphics[width=.9\columnwidth]{moll}
\caption{\label{fig:apx:moll}The base approximation $\fhN$ is transformed into the mollified
approximation $\fhlN$ by replacing Dirac deltas $\delta$ with the mollified deltas $\deltal$.}
\end{figure}

\subsection{Main Result}
Let us define $E(x):=\|\,[x_1\ \cdots\ x_n\ 1]\,\|_2=\|X\|_2$ as the Euclidean norm mapping from 
$\R^n\times\{1\}$ to $\R$, and then define
\begin{equation}\label{eq:apx:EB}
%\Esup := \normSupB{E(x)}
%\qquad\text{and}\qquad
\EB := \normB{E(x)}
\end{equation}
as the $L_2(\Bc,\muB)$ norm of this mapping over the Euclidean distances of $x\in\Bc$. We can now
state the main result, which bounds the difference between a base approximation and its 
corresponding mollified approximation, for a chosen mollifcation factor $\lambda$, in the 
$L_2(\Bc,\muB)$ norm.

\begin{theorem}\label{thm:apx:moll}
\textit{
Let there exist a base approximation $\fhN$ of the form \eqref{eq:apx:baseApx} using any 
activation function $\sigma$ satisfying Assumption~\ref{sigAsmpt}, for any $N\in\N$, with some 
unknown parameters $\upgamma_1,\dots,\upgamma_N\in\Upsilon$ and coefficients $\theta\in\R^N$, 
but having a known bound on the coefficient size of $\sum_{i=1}^N|\theta_i|\leq \Sc_N$ and the 
parameters set $\Upsilon$ known. Then, the mollified approximation $\fhlN$ over the 
$\lambda$-expanded parameters set $\Upsilonl$ in \eqref{eq:apx:mollApx} satisfies either of:}
\begin{align}\label{eq:apx:epslSupBound}
i)\hspace{55.5pt} \normB{\fhN-\fhlN} \ &\leq \ \Sc_N \, \Dsig \\\label{eq:apx:epslL2Bound}
ii)\hspace{52pt} \normB{\fhN-\fhlN} \ &\leq \ \Sc_N\, \frac{\Lsig\,\sqrt{n+1}}{\lambda}\ \EB \ .
\end{align}
\end{theorem}
\begin{proof}
\if\ARXIV1
Given in Appendix~\ref{app:apx:mollProof}.
\fi
\if\ARXIV0
Given in Appendix I of \cite{lekang2023functionfull}.
\fi
\end{proof}

\begin{remark}
The results of Theorem~\ref{thm:apx:moll} show that if the activation function $\sigma$ is 
Lipschitz over its feasible inputs, then as $\lambda\to\infty$ we have $\fhlN(x)\to\fhN(x)$ in 
the sense of the $L_2(\Bc,\muB)$ norm.
\end{remark}

==> random.tex <==
\section{Randomly Initialized Approximations}
\label{sec:apx:random}

In this section, we focus on random approximations $\fhR$ of the form \eqref{eq:apx:rndApx} and 
show that they exist (in high probability) with approximation error in the 
$L_2\left(\Bc,\muB\right)$ norm 
of the shape $O(\frac{1}{\sqrt{R}})$, down to the equivalent bound $\epsbase$ as in 
\eqref{eq:apx:normBound} of an existing base approximation $\fhN$ as in \eqref{eq:apx:baseApx}.

This is done by creating the corresponding mollified approximation $\fhlN$, which has a 
mollified integral representation and therefore can be approximated with randomly sampled 
parameters, which gives $\fhR$.

\begin{figure}[H]
\centering
\begin{tikzpicture}[node distance=1.5em,
        nodes={draw,fill=white},
        box/.style={align=left,inner sep=1ex},
        marrow/.style={single arrow,
              single arrow head extend=1mm,
              execute at begin node={\strut}}]
   \node (A) [box] {$\fhN$ };
   \node (B) [box, right=of A] {$\fhlN$};
   \node (C) [box, right=of B] {$\fhR$};
\draw [->] (A) edge (B) (B) edge (C);
\end{tikzpicture}
%\caption{\label{fig:apx:apxBlock} XXXX.}
\end{figure}

\subsection{Expected Value of Random Approximations to Functions with Integral Representations}

An important property of functions that have integral representations with some activation 
$\sigma$ is that random approximations $\fhR$ of the form \eqref{eq:apx:rndApx} exist which are
exactly equal to the function in expected value over the randomly drawn parameters.

And so, the following lemma builds upon the mollified integral representation of the mollified
approximation $\fhlN$ to show that there always exists random approximations with randomly 
sampled parameters from the $\lambda$-expanded set $\Upsilonl$ satisfying this property.

\begin{lemma}\label{lem:apx:exp}
\textit{
Let the target function $f\in\Cs(\Bc)$ satisfy Theorem~\ref{thm:apx:moll} and thus have the
mollified approximation $\fhlN$ as in \eqref{eq:apx:intRep} with activation $\sigma$ for the 
selected mollification factor $\lambda>0$, which has the integral representation
\eqref{eq:apx:baseIntRepLam} over the $\lambda$-expanded parameters set $\Upsilonl$.
If the random parameters $\upgammab_1,\dots,\upgammab_R$ are sampled iid according
to any density $\Pl$ which is nonzero over $\Upsilonl$, then there exists a random approximation
$\fhR$ of the form \eqref{eq:apx:rndApx} using the activation $\sigma$ such that}
\begin{equation}\label{eq:apx:expL}
\Exp_{\upgammab_j\sim\Pl}\limits\left[\fhR(x\,;\upgammab_1,\dots,\upgammab_R)\right] \
= \ \fhlN(x)
% \hspace{40pt} \forall x\in\Bc 
\ .
\end{equation}
\end{lemma}
\begin{proof}
\if\ARXIV1
Given in Appendix~\ref{app:apx:exp}.
\fi
\if\ARXIV0
Given in Appendix II of \cite{lekang2023functionfull}.
\fi
\end{proof}
\textit{Proof Sketch:} Let us first make the following definitions. With $\gl(\upgamma)$ as in 
\eqref{eq:apx:gLam} for any $\lambda>0$, we define
\begin{align}
%\nonumber
%\gl(\upgamma)& = \sum_{i=1}^N\theta_i\,\deltalno(\upgamma-\upgamma_i) \ \implies 
%\\
\label{eq:apx:Cgl}
&\max_{\upgamma\in\Upsilonl}\limits|\gl(\upgamma)| \ \leq \ 
\sum_{i=1}^N|\theta_i|\left(\frac{\eta\lambda}{e}\right)^{n+1} \ =:\ \Cgl \ .
\end{align}
For the corresponding $\Upsilonl$, we define the diameter $\Dt:=\sup\{\|\upgamma-\phi\|_2 \ | \ 
\upgamma,\phi\in\Upsilonl\}$ and largest point $\upmax:=\sup\{\|\upgamma\|_2 \ | \ 
\upgamma\in\Upsilonl\}$, and for the selected $\Pl$ we define the minimum  $\pmin := 
\inf\{\Pl(\upgamma) \ | \ \upgamma\in\Upsilonl\}$.

Then, note that the RHS of \eqref{eq:apx:mollApx} is equivalently
%\eqref{eq:apx:intRep} can be equivalently expressed in terms of an expectation, as
%\label{eq:apx:intRep2}
\begin{align*}
&\fhlN(x) \ = \\
&\int_\Upsilonl \frac{\gl(\upgamma)}{\Pl(\upgamma)}\,\sigma(\upgamma^\top z)
\,\Pl(\upgamma)\d\upgamma
= \Exp_{\upgammab\sim\Pl}\limits
\left[\frac{\gl(\upgammab)}{\Pl(\upgammab)}\,\sigma(\upgammab^\top z)\right]
%\hspace{40pt} \forall x\in\Bc
\ .
\end{align*}

Thus, a random approximation $\fhR$ exists which satisfies \eqref{eq:apx:expL} by setting its 
coefficients, for all $j\in[R]$, as
\begin{equation*}\label{eq:appApx:cjOpt}
\vartheta_j = \frac{\gl(\upgammab_j)}{\Pl(\upgammab_j)\,R}
\ =\ \frac{\sum_{i=1}^N\theta_i\,\deltalno(\upgammab_j-\upgamma_i)}{\Pl(\upgammab_j)\,R}
\ \ .
\end{equation*}


\subsection{Random Approximations to Base Approximations}
\label{sec:apx:main}

We now state and prove an overall bound on the approximation error in $L_2(\Bc,\muB)$ norm, 
between a base approximation $\fhN$ of the form \eqref{eq:apx:baseApx} to a target function 
$f\in \Cs(\Bc)$ and a random approximation $\fhR(x\,;\upgammab_1,\dots,\upgammab_R)$ of the form 
\eqref{eq:apx:rndApx}.

\begin{theorem}\label{thm:apx:main}
\textit{
Let there exist a base approximation $\fhN$ of the form \eqref{eq:apx:baseApx}, for some integer 
$N\in\N$, to a target function $f\in \Cs(\Bc)$, with unknown parameters 
$\upgamma_1,\dots,\upgamma_N$ in a known bounded parameter set $\Upsilon\subset\R^{n+1}$, 
unknown coefficients $\theta\in\R^N$ with a known bound on the coefficient size
$\sum_{i=1}^N|\theta_i|\leq\Sc_N$, and using an activation function $\sigma$ satisfying
Assumption~\ref{sigAsmpt}. Assume that $\normB{\fch(x)-\fhN(x)}\leq\epsbase$ holds for some 
$\epsbase>0$ which may depend on $N$, for an affine shift $\fch(x)=f-\as^\top\!x-\bs f(0)$ with
some $\as\in\R^n$ and $\bs\in\R$.
The mollified approximation $\fhlN$ as in \eqref{eq:apx:mollApx}
satisfies the results of Theorem~\ref{thm:apx:moll} for any mollification factor $\lambda>0$.
Let the random parameters $\upgammab_1,\dots,\upgammab_R$ be sampled iid according to any
nonzero density $\Pl$ over the $\lambda$-expanded set $\Upsilonl$, which has diameter $\Dt$ and
farthest point $\upmax$, and let $\EB$ be as in \eqref{eq:apx:EB}. Then for any $\nu\in(0,1)$,
with probability greater than $1-\nu$ there exists a random approximation 
$\fhR(x\,;\upgammab_1,\dots,\upgammab_R)$ as in \eqref{eq:apx:rndApx} with
$|\vartheta_j|\leq\frac{\Cgl}{\pmin R}$ for all $j\in[R]$ such that either of the following 
hold:}
\begin{align*}
&\normB{\,\fch(x) - \fhR(x\,;\upgammab_1,\dots,\upgammab_R)} \ \leq \\
&i)\hspace{34pt}
\epsbase + 
\Sc_N\Dsig\left(1 \ + \ 
\frac{\lambda^{n+1}}{\sqrt{R}\,}\,\KD(\nu)\right) \\
&ii)\hspace{30pt}
\epsbase + 
\Sc_N\Lsig\left(\frac{\sqrt{n+1}}{\lambda}\,\EB +
\frac{\lambda^{n+1}}{\sqrt{R}\,}\,\KL(\nu)\right) \ \  .
\end{align*}
The coefficients $\KD$ and $\KL$ are defined in terms of the selected $\nu$ as:
\begin{align*}
&\KD(\nu) \ := \ 
\frac{\eta^{n+1}}{e^{n+1}\pmin}
\left(
1 + \frac{|\sigma(0)|}{\Dsig} \right. \\
&\left. + \bigg(3 + 2\frac{|\sigma(0)|}{\Dsig}\bigg) 
\sqrt{\frac{1}{2}\log\left(\frac{1}{\nu}\right)}
\right) \\
&\KL(\nu) \ := \
\frac{\eta^{n+1}}{e^{n+1}\pmin}
\left(
\upmax\EB + \frac{|\sigma(0)|}{\Lsig}\right. \\
&\left. + \bigg((\Dt+2\upmax)\EB + 
2\frac{|\sigma(0)|}{\Lsig}\bigg) \sqrt{\frac{1}{2}\log\left(\frac{1}{\nu}\right)}
\right).
\end{align*}
\end{theorem}
\begin{proof}
\if\ARXIV1
Given in Appendix~\ref{app:apx:mainProof}.
\fi
\if\ARXIV0
Given in Appendix II of \cite{lekang2023functionfull}.
\fi
\end{proof}
\textit{Proof Sketch:} We closely follow the strategy in Lemma 4 of
\cite{rahimi2008weighted}, which uses McDiarmid's inequality to obtain the final result.

We start by defining function $h_\Bc:\Upsilon^R_\lambda\to\R$, which captures the norm difference
between the random approximation and its expected value over the iid draws of 
$(\upgammab_1,\dots,\upgammab_R)\in\Upsilon^R_\lambda$, as
\begin{align}
\label{eq:apx:hB}
&h_\Bc(\upgammab_1,\dots,\upgammab_R) \ := \\\nonumber
&\normB{\,\fhR(x\,;\upgammab_1,\dots,\upgammab_R)
-\Exp_{\upgammab_j\sim\Pl}\limits\left[\fhR(x\,;\upgammab_1,\dots,\upgammab_R)\right]} \ \ .
\end{align}
Thus, we can use Lemma~\eqref{lem:apx:exp} to show that there exists $\fhR$ such that 
\eqref{eq:apx:hB} is equivalently
$$
h_\Bc(\upgammab_1,\dots,\upgammab_R) \ = \ \normB{\,\fhlN(x) - 
\fhR(x\,;\upgammab_1,\dots,\upgammab_R)} \ .
$$
We then can bound the expected value
$$
\Exp_{\upgammab_j\sim\Pl}\limits\Big[h_\Bc(\upgammab_1,\dots,\upgammab_R)\Big]
$$
and the absolute value of the difference between any 
$$
\big|h_\Bc(\upgamma_1,\dots,\upgamma_j,\dots,\upgamma_R)-
h_\Bc(\upgamma_1,\dots,\widetilde\upgamma_j,\dots,\upgamma_R)\big|
$$
that differ only at one coordinate, over each $j\in[R]$. These two bounds then allow us to apply 
the results of McDiarmid's inequality, thus bounding (in high probability)
$$
\normB{\,\fhlN(x) - 
\fhR(x\,;\upgammab_1,\dots,\upgammab_R)} \ .
$$
The proof is then completed by using the triangle inequality, with
\begin{align*}
&\normB{\,\fch(x) - \fhR(x\,;\upgammab_1,\dots,\upgammab_R)} \ \leq \ 
\normB{\fch(x)-\fhN(x)} +\\ &\ \normB{\fhN(x)-\fhlN(x)} 
+\normB{\fhlN(x)-\fhR(x\,;\upgammab_1,\dots,\upgammab_R)} \ .
\end{align*}
where the first term is assumed bounded by $\epsbase$ for the base approximation $\fhN$ and the 
second term is bounded by Theorem~\ref{thm:apx:moll}.

\begin{remark}
Classic results from \cite{barron1993universal} and \cite{breiman1993hinging} prove the existence
of \textit{convex} combinations of step \eqref{eq:pe:step} and ReLU \eqref{eq:pe:ReLU} 
activations that approximate (affine shifts of) functions in specific classes arbitrarily well, 
with an 
approximation error proportional to $\epsbase=O\left(\frac{1}{\sqrt{N}}\right)$. Importantly, 
the 
convexity property allows the length (number
of terms) $N$ to be arbitrarily large while maintaining the same overall bound on the 
coefficient size $\sum_{i=1}^N|\theta_i|\leq\Sc_N$.
This means we can allow the number of terms to grow 
arbitrarily large $N\to\infty$, since $N$ does not appear directly in the results of 
Theorem~\ref{thm:apx:main}. This gives $\epsbase\to0$, while maintaining the same bound $\Sc_N$.
\end{remark}

